Exploring Parameter-Efficient Fine-Tuning Techniques for Code Generation with Large Language Models

Large language models (LLMs) demonstrate impressive capabilities to generate accurate code snippets given natural language intents in a zero-shot manner, i.e., without the need for specific fine-tuning. While prior studies have highlighted the advantages of fine-tuning LLMs, this process incurs high computational costs, making it impractical in resource-scarce environments, particularly for models with billions of parameters. To address these challenges, previous research explored in-context learning (ICL) and retrieval-augmented generation (RAG) as strategies to guide the LLM generative process with task-specific prompt examples. However, ICL and RAG introduce inconveniences, such as the need for designing contextually relevant prompts and the absence of learning task-specific parameters, thereby limiting downstream task performance. In this context, we foresee parameter-efficient fine-tuning (PEFT) as a promising approach to efficiently specialize LLMs to task-specific data while maintaining reasonable resource consumption. In this paper, we deliver a comprehensive study of PEFT techniques for LLMs in the context of automated code generation. Our comprehensive investigation of PEFT techniques for LLMs reveals their superiority and potential over ICL and RAG across a diverse set of LLMs and three representative Python code generation datasets: Conala, CodeAlpacaPy, and APPS. Furthermore, our study highlights the potential for tuning larger LLMs and significant reductions in memory usage by combining PEFT with quantization. Therefore, this study opens opportunities for broader applications of PEFT in software engineering scenarios. Our code is available at https://github.com/martin-wey/peft-llm-code/.

==> content/5_results_backup.tex <==
\section{Experimental Results}
\label{sec:experimental-results}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/rq1_icl.pdf}
    \caption{\martin{New figure RQ1}}
    \label{fig:enter-label}
\end{figure}

\input{tables/rq1}

\subsection{RQ1: Performance Exploration Based on Model Size and Tuning Technique}
\label{sec:rq1_results}

We report the detailed results of the performance of the small language models and LLMs on code generation for both CoNaLa and CodeAlpacaPy datasets in Table~\ref{tab:RQ1}. 

\subsubsection*{Small models vs. LLMs} 
CodeGen-350M-mono with LoRA demonstrates the best performance on average among small models, while CodeLlama-7B-Python with LoRA is the best LLM on average. 
Under the same 24GB GPU memory limitation, the best LLM surpasses the best small model by 39.8\%, 41.7\%, and 47.1\% (72.3\%, 48.8\%, and 9.1\%) in EM@1, EM@10, and CodeBLEU concerning the CoNala (CodeAlpacaPy) dataset, respectively. These notable results indicate a potential shift towards a new era of LLMs, differing from the popular paradigm in the SE community over the past 3-4 years: fine-tuning small pre-trained models such as CodeT5.

\subsubsection*{Small language models}
Among the small language models, CodeGen-350M-mono shows the highest effectiveness across all metrics on both datasets. 
Our results align with prior studies~\cite{zhou2023docprompting, wang2022execution, nijkamp2023codegen} that identified CodeGen-350M-mono as a robust small language model for Python code generation tasks. Interestingly, although it requires tuning approximately 1\% of the total parameters of the model, LoRA appears as the best tuning technique, surpassing full fine-tuning by a considerable margin across nearly all configurations. 
For instance, the EM@10 score for CodeGen-350M-mono on the CoNaLa dataset, with full fine-tuning, is 18.42, while it soars to 25.60 with LoRA.

\subsubsection*{LLMs} 
In Figure~\ref{fig:rq1_scatter_plots}, we present a comparative analysis of the models' effectiveness when tuned using LoRA, focusing on CodeBLEU and EM@10 scores. 
Both plots clearly establish CodeLlama-7B models as the best-performing LLMs in our study.
Remarkably, CodeGen2-7B, despite sharing a similar number of parameters, lags behind all CodeLlama-7B variants.
Unsurprisingly, harnessing larger models leads to better effectiveness.
Given the low computational costs of PEFT techniques, leveraging smaller models in a context akin to ours seems counterproductive.
Subsequently, in this paper, we demonstrate that even larger models can be fine-tuned through the combination of PEFT with quantization.

\subsubsection*{Best PEFT technique}
Overall, LoRA emerges as the most effective PEFT technique among the studied ones. 
Although being presented as an incremental improvement over LoRA~\cite{liu2022few}, IA3 often shows lower scores compared to LoRA.
Prompt tuning appears as another viable tuning option, while further reducing the number of trainable parameters. 
However, Prefix tuning fails to effectively adapt the larger models to both datasets.

Our analysis reveals notably higher EM scores for the CoNaLa dataset, which can be attributed to differences in task complexity between the two datasets (see Section~\ref{sec:dataset_task}).
It is important to note that CodeBLEU scores on CoNala are comparatively lower due to the metric's reliance on dataflow graph computations, which may not always be available for small code examples.

\begin{tcolorbox}[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,
borderline west={1mm}{0pt}{blue!50!white},colback=blue!10!white]
 \textbf{Answer to RQ1}: LLMs with PEFT consistently and significantly outperform small language models under the same GPU limit.
 Specifically, the best-performing LLM with PEFT surpasses the best small model by 39.8--72.3\% in terms of EM@$k$.
 Among different PEFT techniques, LoRA is the most effective one.
\end{tcolorbox}

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/rq2_conala.pdf}
  \caption{CoNaLa}
  \label{fig:rq1_scatter_conala}
\end{subfigure}%
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/rq2_codealpaca.pdf}
  \caption{CodeAlpacaPy}
  \label{fig:rq1_scatter_codealpaca}
\end{subfigure}
\caption{[RQ1] -- Effectiveness of the models fine-tuned using LoRA for both datasets in terms of EM@10 and CodeBLEU.}
\label{fig:rq1_scatter_plots}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.8\linewidth]{figures/rq2_lora_vs_icl.pdf}
    \vspace{-1em}
    \caption{[RQ2] -- Comparison of the effectiveness of the models using LoRA and ICL on CoNaLa (top) and CodeAlpacaPy (bottom). \martin{RQ2 updated}}
    \label{fig:rq2_lora_vs_icl}
\end{figure}

\subsection{RQ2: Comparative Study Between PEFT and ICL Applications}
\label{sec:rq2_results}

In this RQ, we aim to investigate whether PEFT techniques in RQ1 consistently outperform the widely used ICL when applying LLMs in code generation.
In Figure~\ref{fig:rq2_lora_vs_icl}, we compare the effectiveness of the small language models and LLMs using ICL and LoRA in terms of CodeBLEU and EM@10.
Note that for the CodeAlpacaPy dataset, we do not report CodeGen2 models' ICL performance as the increase in the prompt size induced dramatic inference latency for this family of models.
For ICL, we compute the average metrics obtained over five random seeds, with up to 3 prompt examples.
We report in Figure~\ref{fig:rq2_lora_vs_icl} the highest metrics achieved over the different ICL configurations for each model.

\subsubsection*{ICL effectiveness}
A notable performance gap exists between CoNala and CodeAlpacaPy datasets, as illustrated in Figure~\ref{fig:rq2_lora_vs_icl}. CodeAlpacaPy, in particular, poses significant challenges, emphasizing the undeniable necessity of employing PEFT for adapting LLMs to such a dataset.
Across both datasets, CodeLlama-7B models demonstrate substantially higher effectiveness compared to other models.
For example, CodeLlama-7B-Python shows impressive performance on CoNala with 29.47 in EM@10 and 23.90 in CodeBLEU, without any fine-tuning. 
In contrast, CodeGen2-7B achieves lower results, with 24.49 in EM@10 and 17.73 in CodeBLEU.

\subsubsection*{LoRA vs. ICL}
LoRA significantly enhances model performance for both datasets compared to ICL. 
Notably, CodeLlama-7B-Python, with LoRA tuning, enhances EM@10 and CodeBLEU by 23.1\% over ICL on CoNala.
This trend extends to CodeAlpacaPy, with higher relative gains in EM@$k$.
For instance, CodeLlama-7B-Python increases EM@10 by 178\% and CodeBLEU by 19.2\% with LoRA over ICL.
On average, LLMs tuned using LoRA improve by 25.4\% and 22.8\% (150\% and 29.8\%) in EM@10 and CodeBLEU concerning the CoNaLa (CodeAlpacaPy) dataset, respectively.
Overall, PEFT presents only advantages over ICL as it considerably improves the effectiveness of all the studied models without requiring the selection of ICL examples during inference, prompting future research to consider PEFT over ICL.

\begin{tcolorbox}[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,
borderline west={1mm}{0pt}{blue!50!white},colback=blue!10!white]
 \textbf{Answer to RQ2}: PEFT techniques outperform ICL as they consistently enhance the effectiveness of all the models.
 LLMs tuned using LoRA improves by 25.4\% and 22.8\% (150\% and 29.8\%) in EM@10 and CodeBLEU concerning the CoNaLa (CodeAlpacaPy) dataset, respectively.
\end{tcolorbox}

\begin{comment}
\subsection{RQ3: Joint Training with a Single LoRA Adapter}
\label{sec:rq3_results}

In Table~\ref{tab:RQ3}, we report a comparative analysis of the models' effectiveness when fine-tuned with LoRA on both datasets separately versus a joint training approach where the datasets are concatenated for fine-tuning.
The key advantage of the joint training approach is that it leverages a single LoRA adapter for learning and encoding knowledge from both datasets.
In contrast, the former method requires a dedicated adapter for each dataset.

Our analysis reveals that both approaches exhibit only minimal disparities in the evaluation metrics across all models.
In certain instances, the joint training approach surpasses the single-dataset approach, with only marginal variations in the metrics.
For example, both approaches demonstrate comparable effectiveness when applied to CodeLlama-7B-Python, underscoring the benefits of the joint training strategy, which obviates the need for relying on multiple adapters during inference.

\begin{tcolorbox}[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,
borderline west={1mm}{0pt}{blue!50!white},colback=blue!10!white]
 \textbf{Answer to RQ3}: Our analysis reveals no substantial disparities between the joint training and single-dataset approaches.
 This suggests that the joint training approach with LoRA is an effective way of adapting the LLMs on both datasets and thus performing inference using a single adapter.
\end{tcolorbox}
\end{comment}

\subsection{RQ4: Investigation of the Tuning of CodeLlama Models with QLoRA}
\label{sec:rq4_results}
In this final experiment, we exploit the benefits of QLoRA~\cite{dettmers2023qlora}, a computationally efficient technique that combines LoRA with quantization for fine-tuning LLMs.
QLoRA employs 8-bit or 4-bit quantization during fine-tuning, reducing memory usage by lowering the precision of the model's weights.
Our objectives are to showcase the substantial memory reduction achieved by QLoRA for LLMs and underscore its ability to facilitate fine-tuning of larger models with limited computing resources.

In Figure~\ref{fig:rq4}, we display EM@10 scores for three CodeLlama model variants: CodeLlama-7B-Python, CodeLlama-13B-Python, and CodeLlama-34B, alongside peak GPU memory consumption consistently below 24GB for each tuning configuration.
CodeBLEU scores are not reported due to similar observed trends.
We fine-tuned the models using LoRA and QLoRA, with 8-bit (QLoRA-8bit) and 4-bit (QLoRA-4bit) quantization. 
We only use QLoRA-8/4-bit for CodeLlama-13B-Python, and QLoRA-4bit for CodeLlama-34B-Python to avoid memory overflow. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=.9\linewidth]{figures/rq4_qlora_vs_lora.pdf}
    \vspace{-1em}
    \caption{[RQ2.2] -- Performance of CodeLlama models using LoRA and QLoRA with 8-bit and 4-bit quantization. %The cost of all the assessed techniques and models remains within the limit of our constrained computational budget.
    }
    \label{fig:rq4}
\end{figure*}

\subsubsection*{Performance of the LLMs}
The results underscore a significant improvement in the effectiveness of larger quantized models on both datasets, with a more moderate impact on CodeAlpacaPy.
For instance, CodeLlama-34B-Python, fine-tuned with QLoRA-4bit, achieves a substantial 12.2\% increase in CoNaLa's EM@10 score (40.70) compared to CodeLlama-7B-Python with LoRA (36.28). 
Surprisingly, QLoRA also brings notable improvements over LoRA for CodeLlama-7B-Python on CoNaLa, while achieving comparable results on CodeAlpacaPy.
Moreover, QLoRA-4bit exhibits further enhancements in EM@10 compared to QLoRA-8bit for this model.

\subsubsection*{Computational gains}
Both QLoRA-8bit and QLoRA-4bit substantially reduce memory usage.
Specifically, for CodeLlama-7B-Python, QLoRA-4bit achieves a remarkable 2x reduction in peak memory usage while significantly improving the EM@10 score.
The application of quantization enables the utilization of larger models that can be accommodated within a single 24GB GPU.
Notably, throughout the fine-tuning and inference processes, we did not observe substantial latencies, affirming the practical feasibility of leveraging such models without compromising computational efficiency.

\begin{tcolorbox}[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,
borderline west={1mm}{0pt}{blue!50!white},colback=blue!10!white]
 \textbf{Answer to RQ4}: QLoRA reduces memory usage, achieving up to a 2-fold decrease compared to LoRA, all while preserving or even improving the model's effectiveness across both CoNaLa and CodeAlpacaPy datasets.
 Furthermore, QLoRA facilitates the fine-tuning of LLMs with up to 34B parameters.
\end{tcolorbox}



==> tables/rq1_backup.tex <==
\renewcommand{\arraystretch}{.9}
\setlength{\arrayrulewidth}{.5pt}
\setlength\extrarowheight{.5pt}
\setlength\dashlinedash{2pt}
\setlength\dashlinegap{2pt}
\begin{table}[!t]
\centering
\footnotesize
\caption{[RQ1] -- Comparison of the small language models and LLMs using various tuning techniques (bold: best-performing PEFT per model, underlined: best-performing model).} 
\label{tab:RQ1}
\vspace{-1em}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{llr*{6}{>{\centering\arraybackslash}p{1cm}}*{6}{c}}
    \toprule
    &  &  & \multicolumn{3}{c}{CoNaLa} & \multicolumn{3}{c}{CodeAlpacaPy} \\ 
    \cmidrule(l{1em}r{1em}){4-6} \cmidrule(l{1em}r{1em}){7-9}
    Model & Tuning & \# Params & EM@1 & EM@10 & CodeBLEU & EM@1 & EM@10 & CodeBLEU \\ 
    \midrule
    % \multicolumn{9}{c}{\cellcolor{blue!25} \normalsize Small LMs} \\
    % \midrule
    \arrayrulecolor{black!50}
    
    \multirow{5}{*}{CodeT5+-220M} & Full FT & 220M & \color{black!50} 3.87 & \color{black!50} 8.84 & \color{black!50} 16.70 & \textbf{3.98} & \textbf{7.64} & \textbf{25.49} \\
    
    & LoRA & 2.7M  & \textbf{6.08} & \textbf{12.71} & \textbf{18.96} & \color{black!50} 3.34 & \color{black!50} 5.26 & \color{black!50} 24.32 \\
    
    & IA3 & 0.17M & \color{black!50} 4.42 & \color{black!50} 10.68 & \color{black!50} 17.08 & \color{black!50} 0.64 & \color{black!50} 1.27 & \color{black!50} 22.06 \\
    
    & Prompt tuning & 0.03M & \color{black!50} 4.79 & \color{black!50} 9.21 & \color{black!50} 16.30 & \color{black!50} 0.96 & \color{black!50} 2.07 & \color{black!50} 19.01 \\
    
    & Prefix tuning & 0.18M & \color{black!50} 3.13 & \color{black!50} 7.55 & \color{black!50} 14.56 & \color{black!50} 0.16 & \color{black!50} 1.27 & \color{black!50} 20.80 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{5}{*}{CodeT5+-770M} & Full FT & 770M & \color{black!50} 4.05 & \color{black!50} 8.29 & \color{black!50} 15.11 & \color{black!50} 3.19 & \color{black!50} 6.21 & \color{black!50} 27.73 \\
    
    & LoRA & 7M & \textbf{8.66} & \color{black!50} 17.13 & \textbf{20.64} & \textbf{3.66} & \textbf{6.85} & \textbf{26.10} \\
    
    & IA3 & 0.4M  & \color{black!50} 8.10 & \textbf{17.50} & \color{black!50} 18.68 & \color{black!50} 2.87 & \color{black!50} 5.26 & \color{black!50} 25.84 \\
    
    & Prompt tuning & 0.04M & \color{black!50} 7.37 & \color{black!50} 15.47 & \color{black!50} 16.75 & \color{black!50} 1.91 & \color{black!50} 3.82 & \color{black!50} 20.57 \\
    
    & Prefix tuning & 0.5M & \color{black!50} 4.97 & \color{black!50} 11.97 & \color{black!50} 16.77 & \color{black!50} 0.16 & \color{black!50} 1.27 & \color{black!50} 22.91 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{5}{*}{CodeGen-350M-mono} & Full FT & 350M & \color{black!50} 7.92 & \color{black!50} 18.42 & \color{black!50} 14.68 & \color{black!50} 2.23 & \color{black!50} 5.73 & \color{black!50} 21.78 \\
    
    & LoRA & 1.3M & \textbf{12.52} & \color{black!50} 25.60 & 
    \color{black!50} 17.89 & \textbf{4.62} & \textbf{10.70} & \textbf{30.09} \\
    
    & IA3 & 0.16M & \color{black!50} 11.42 & \textbf{25.78} & \textbf{18.83} & \color{black!50} 4.46 & \textbf{10.70} & \color{black!50} 28.56 \\
    
    & Prompt tuning & 0.02M & \color{black!50} 7.92 & \color{black!50} 20.26 & \color{black!50} 16.29 & \color{black!50} 0.0 & \color{black!50} 0.0 & \color{black!50} 25.91 \\
    
    & Prefix tuning & 0.4M & \color{black!50} 5.34 & \color{black!50} 12.52 & \color{black!50} 17.53 & \color{black!50} 0.0 & \color{black!50} 0.0 & \color{black!50} 26.89 \\
    
    \midrule
    
    \multirow{4}{*}{CodeGen2-1B} & LoRA & 2M & 
    \color{black!50} 9.39 & \textbf{23.02} & \textbf{19.76} & \textbf{3.82} & \color{black!50} 9.08 & \color{black!50} 23.48 
    \\
    
    & IA3 & 0.2M & \color{black!50} 10.13 & \color{black!50} 22.84 & \color{black!50} 18.64 & \textbf{3.82} & \textbf{9.87} & \textbf{24.42} \\
    
    & Prompt tuning & 0.04M & \textbf{11.97} & \color{black!50} 22.65 & \color{black!50} 18.38 & \color{black!50} 0.80 & \color{black!50} 2.07 & \color{black!50} 18.17 \\
    
    & Prefix tuning & 0.6M & \color{black!50} 5.89 & \color{black!50} 15.84 & \color{black!50} 18.46 & \color{black!50} 0.0 & \color{black!50} 0.32 & \color{black!50} 13.68 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{4}{*}{CodeGen2-3.7B} & LoRA & 4M & \textbf{11.60} & \color{black!50} 25.97 & \color{black!50} 19.00 & \textbf{5.41} & \color{black!50} 10.70 & \color{black!50} 23.75 \\
    
    & IA3 & 0.5M & \color{black!50} 10.87 & \color{black!50} 25.23 & \color{black!50} 19.21 & \textbf{5.41} & \textbf{10.99} & \textbf{26.26} \\
    
    & Prompt tuning & 0.08M & \color{black!50} 11.05 & \textbf{26.89} & \color{black!50} 19.53 & \color{black!50} 0.0 & \color{black!50} 0.0 & \color{black!50} 23.42 \\
    
    & Prefix tuning & 1.3M & \color{black!50} 10.68 & \color{black!50} 24.68 & \textbf{20.23} & \color{black!50} 0.16 & \color{black!50} 0.32 & \color{black!50} 21.73 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{4}{*}{CodeGen2-7B} & LoRA & 8.3M & \color{black!50} 11.23 & \textbf{29.83} & \textbf{23.86} & \color{black!50} 5.57 & \color{black!50} 11.94 & \color{black!50} 27.73 \\
    
    & IA3 & 1M & \color{black!50} 11.42 & \color{black!50} 29.65 & \color{black!50} 21.98 & \textbf{5.73} & \textbf{12.42} & 
    \textbf{28.26} \\
    
    & Prompt tuning & 0.08M & \textbf{11.97} & \color{black!50} 27.26 & \color{black!50} 22.37 & \color{black!50} 0.0 & \color{black!50} 0.0 & \color{black!50} 25.40 \\
    
    & Prefix tuning & 2.6M & \color{black!50} 9.95 & \color{black!50} 23.94 & \color{black!50} 22.29 & \color{black!50} 0.0 & \color{black!50} 0.32 & \color{black!50} 25.72 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{4}{*}{CodeLlama-7B} & LoRA & 12.5M & \textbf{\underline{20.07}} & \textbf{\underline{39.31}} & \textbf{25.33} & \color{black!50} 7.33 & \textbf{16.24} & \textbf{32.05} \\
    
    & IA3 & 1M & \color{black!50} 17.68 & \color{black!50} 37.20 & \color{black!50} 23.19 & \textbf{8.12} & \color{black!50} 15.45 & \color{black!50} 30.47 \\
    
    & Prompt tuning & 0.08M & \color{black!50} 19.15 & \color{black!50} 38.12 & \color{black!50} 25.01 & \color{black!50} 0.32 & \color{black!50} 0.48 & \color{black!50} 31.55 \\
    
    & Prefix tuning & 2.6M & \color{black!50} 8.47 & \color{black!50} 19.52 & \color{black!50} 23.19 & \color{black!50} 0.16 & \color{black!50} 0.16 & \color{black!50} 28.09 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{4}{*}{CodeLlama-7B-Instruct} & LoRA & 12.5M & \color{black!50} 17.68 & \textbf{36.28} & \color{black!50} 24.27 & \color{black!50} 7.01 & \textbf{\underline{17.04}} & \textbf{31.42} \\
    
    & IA3 & 1M & \color{black!50} 15.84 & \color{black!50} 36.10 & \color{black!50} 24.71 & \textbf{8.12} & \color{black!50} 16.72 & \color{black!50} 31.01 \\
    
    & Prompt tuning & 0.08M & \textbf{18.97} & \color{black!50} 35.54 & \textbf{25.77} & \color{black!50} 1.59 & \color{black!50} 3.50 & \color{black!50} 31.14 \\
    
    & Prefix tuning & 2.6M & \color{black!50} 10.13 & \color{black!50} 18.23 & \color{black!50} 23.66 & \color{black!50} 0.64 & \color{black!50} 0.96 & \color{black!50} 31.27 \\
    
    \cmidrule(l{1em}r{1em}){1-9}
    \multirow{4}{*}{CodeLlama-7B-Python} & LoRA & 12.5M & \textbf{17.50} & \color{black!50} 36.28 & \color{black!50} 24.27 & \color{black!50} 7.96 & \color{black!50} 15.92 & \color{black!50} 32.84 \\
    
    & IA3 & 1M & \color{black!50} 14.55 & \color{black!50} 31.12 & \color{black!50} 24.74 & \textbf{\underline{8.76}} & \textbf{16.56} & \color{black!50} 29.82 \\
    
    & Prompt tuning & 0.08M & \color{black!50} 16.76 & \textbf{37.02} & \textbf{\underline{26.31}} & \color{black!50} 0.96 & \color{black!50} 3.03 & \textbf{\underline{33.46}} \\
    
    & Prefix tuning & 2.6M & \color{black!50} 9.76 & \color{black!50} 22.47 & \color{black!50} 19.47 & \color{black!50} 0.0 & \color{black!50} 0.0 & \color{black!50} 30.71 \\
    \arrayrulecolor{black}
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/rq3_backup.tex <==
\renewcommand{\arraystretch}{0.9}
\setlength{\arrayrulewidth}{.5pt}
\begin{table}[!t]
\centering
\small
\caption{[RQ3] -- Comparison of the models fine-tuned using LoRA and a joint training approach that uses a single LoRA adapter for fine-tuning the models on both datasets.} 
\label{tab:RQ3}
% \vspace{-1em}
\resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{ll|@{\extracolsep{\fill}}*{1}{ccc|ccc}}
    \toprule
     &  & \multicolumn{3}{c}{CoNaLa} & \multicolumn{3}{c}{CodeAlpacaPy} \\ 
    \cmidrule(l{1em}r{1em}){3-5} \cmidrule(l{1em}r{1em}){6-8}
    Model & Tuning & EM@1 & EM@10 & CodeBLEU & EM@1 & EM@10 & CodeBLEU \\
    \midrule
    \arrayrulecolor{black!50}
    CodeT5+-220m & LoRA & \color{black!50} 6.08 & \color{black!50} 12.71 & \textbf{18.96} & \color{black!50} 3.34 & \textbf{5.26} & \color{black!50} 24.32 \\
    CodeT5+-220m & Joint & \textbf{6.63} & \textbf{14.37} & \color{black!50} 17.24 & \textbf{3.66} & \color{black!50} 4.78 & \textbf{24.95} \\
    \midrule
    CodeT5+-770m & LoRA & \color{black!50} 8.66 & \color{black!50} 17.13 & \textbf{20.64} & \textbf{3.66} & \color{black!50} 6.85 & \color{black!50} 26.10 \\
    CodeT5+-770m & Joint & \textbf{10.13} & \textbf{18.42} & \color{black!50} 19.17 & \color{black!50} 3.03 & \textbf{7.01} & \textbf{27.53} \\
    \midrule
    CodeGen-350M-mono & LoRA & \textbf{12.52} & \textbf{25.60} & \color{black!50} 17.89 & \textbf{4.62} & \textbf{10.70} & \textbf{30.09} \\
    CodeGen-350M-mono & Joint & \color{black!50} 11.60 & \color{black!50} 25.23 & \textbf{18.41} & \color{black!50} 4.30 & \color{black!50} 10.29 & \color{black!50} 28.64 \\
    \midrule
    \midrule
    CodeGen2-1B & LoRA & \color{black!50} 9.39 & \textbf{23.02} & \color{black!50} 19.76 & \color{black!50} 3.82 & \textbf{9.08} & \textbf{23.48} \\
    CodeGen2-1B & Joint & \textbf{9.76} & \color{black!50} 22.28 & \textbf{20.92} & \textbf{3.66} & \color{black!50} 8.28 & \color{black!50} 22.54 \\
    \midrule
    CodeGen2-3.7B & LoRA & \color{black!50} 11.60 & \textbf{25.97} & \color{black!50} 19.00 & \textbf{5.41} & \color{black!50} 10.70 & \textbf{23.75} \\
    CodeGen2-3.7B & Joint & \textbf{11.97} & \textbf{25.97} & \textbf{19.76} & \color{black!50} 5.10 & \textbf{11.15} & \color{black!50} 20.98 \\
    \midrule
    CodeGen2-7B & LoRA & \textbf{11.23} & \color{black!50} 29.83 & \textbf{23.86} & \textbf{5.57} & \color{black!50} 11.94 & \color{black!50} 27.73 \\
    CodeGen2-7B & Joint & \color{black!50} 10.31 & \textbf{30.20} & \color{black!50} 22.00 & \color{black!50} 5.26 & \textbf{12.74} & \textbf{28.33} \\
    \midrule
    CodeLlama-7B & LoRA & \textbf{20.07} & \textbf{39.31} & \textbf{25.33} & \color{black!50} 7.33 & \textbf{16.24} & \textbf{32.05} \\
    CodeLlama-7B & Joint & \color{black!50} 17.68 & \color{black!50} 37.20 & \color{black!50} 23.76 & \textbf{7.64} & \color{black!50} 15.13 & \color{black!50} 30.16  \\
    \midrule
    CodeLlama-7B-Instruct & LoRA & \textbf{17.68} & \color{black!50} 36.28 & \textbf{24.27} & \color{black!50} 7.01 & \textbf{17.04} & \textbf{31.42} \\
    CodeLlama-7B-Instruct & Joint & \color{black!50} 16.76 & \textbf{36.65} & \color{black!50} 22.97 & \textbf{7.64} & \color{black!50} 15.92 & \color{black!50} 30.73 \\
    \midrule
    CodeLlama-7B-Python & LoRA & \textbf{17.50} & \color{black!50} 36.28 & \textbf{24.27} & \textbf{7.96} & \textbf{15.92} & \textbf{32.84} \\
    CodeLlama-7B-Python & Joint & \textbf{17.50} & \textbf{37.75} & \color{black!50} 24.09 & \color{black!50} 7.17 & \color{black!50} 15.76 & \color{black!50} 31.40 \\
    \arrayrulecolor{black}
    \bottomrule
    \end{tabular}
    }
\end{table}
